Augmenting text for spoken language understanding with Large Language Models

Spoken semantic parsing (SSP) involves generating machine-comprehensible parses from input speech. Training robust models for existing application domains represented in training data or extending to new domains requires corresponding triplets of speech-transcript-semantic parse data, which is expensive to obtain. In this paper, we address this challenge by examining methods that can use transcript-semantic parse data (unpaired text) without corresponding speech. First, when unpaired text is drawn from existing textual corpora, Joint Audio Text (JAT) and Text-to-Speech (TTS) are compared as ways to generate speech representations for unpaired text. Experiments on the STOP dataset show that unpaired text from existing and new domains improves performance by 2% and 30% in absolute Exact Match (EM) respectively. Second, we consider the setting when unpaired text is not available in existing textual corpora. We propose to prompt Large Language Models (LLMs) to generate unpaired text for existing and new domains. Experiments show that examples and words that co-occur with intents can be used to generate unpaired text with Llama 2.0. Using the generated text with JAT and TTS for spoken semantic parsing improves EM on STOP by 1.4% and 2.6% absolute for existing and new domains respectively.

==> sections/abstract.tex <==










% While TTS is more beneficial for expanding SSP to new application domains, JAT is preferred for efficiency and strong performance when unpaired text is for existing domains. 






% Spoken semantic parsing (SSP) involves extracting machine comprehensible parses from input speech.  Supervised training of such models requires corresponding triplets of speech-transcript-semantic parse data, which is expensive to obtain. In this paper, we address this challenge by developing methods to use only transcript-semantic parse data (unpaired text) without real speech. First, we consider the setting where unpaired textual data can be obtained from existing textual corpora. Joint Audio Text (JAT) and Text-to-Speech (TTS) are compared as ways to generate speech representations for unpaired text. Experiments on the STOP dataset show that additional unpaired text from existing and new domains improves performance by 2 points and 30 points in absolute Exact Match (EM) respectively. While TTS is more beneficial when expanding SSP to new application domains, JAT is preferred for unpaired text from existing domains owing to its simplicity and computational efficiency. Second, we consider the setting when unpaired text is not available in existing textual corpora. Large Language Models (LLMs) can be used to generate transcript-semantic parse data.  Using different prompting strategies with LLama 2.0, we show that such LLM-generated data can be used with JAT and TTS to improve spoken semantic parsing over STOP by 1.4 and 2.6  points in absolute EM for existing and new domains respectively.


% Deliberation-based end-to-end models for SSP use transcript and speech embeddings to generate semantic parses.
%Unlike textual semantic parsing or speech recognition which require pairs of transcript-semantic parse or speech-transcript data, deliberation-based SSP requires triplets of speech-transcript-semantic parse data, which is more expensive to obtain. 

% Of this triplet, transcript-semantic parse pairs can be obtained with relative ease from -- existing textual resources or by prompting Large Language Models (LLMs). This paper explores mechanisms to generate corresponding speech representations for such transcript-text data. First, we compare Text-To-Speech (TTS) and Joint Audio-Text Training (JAT) methods to build speech representations for existing transcript-semantic parse data. We find that synthesis-based approaches are more beneficial when expanding semantic parsing to new domains, while JAT may be preferred for existing domains due to its computational efficiency and comparable performance to TTS. 


% Finally, we use LLama 2.0 to generate synthetic transcript-semantic parse data when such data cannot be obtained from existing resources.


% compares methods to utilize transcript-semantic parse data without corresponding speech when it is available and generate text-semantic parse data when it is not available using Large Language Models (LLMs). 



%This paper aims to develop methods to generate paired speech-transcript-semantic parse using either transcripts or paired transcript-semantic parse data. First, we compare and contrast Text-To-Speech (TTS) and Joint Audio-Text Training (JAT) methods to build speech representations for unpaired text. We find that synthesis based approaches are more beneficial when expanding to new domains, while JAT and TTS confer similar benefits on new data in domains with some amount of real speech. Next, we use LLama 2.0 to generate synthetic text-semantic parse data using different prompting strategies and compare the utility of synthetic data over real data.    Finally, we consider cases when such unpaired data is not readily available, and use the Large Language Model LLaMa 2.0 to generate text and text-semantic parse paired data.  

%Finally, we show that spoken semantic parsers can be trained using a strong speech recognizer and a Large Language Model, without any speech data and paired speech-text-semantic parse data. 

% The higher availability of unpaired text only data for spoken language processing has motivated many approaches to use unpaired text to improve performance. This paper addressed the challenge of using unpaired text for spoken semantic parsing, and compares synthesis-based, decoder-pretraining and joint audio text training approaches. To make this approach more generalizable, this paper then focuses on using large language models to produce contrastive examples and text-only data that is then used to im model performance . 
